SPARSE: Semantic Tracking and Path Analysis for Attack Investigation in Real-time

As the complexity and destructiveness of Advanced Persistent Threat (APT) increase, there is a growing tendency to identify a series of actions undertaken to achieve the attacker's target, called attack investigation. Currently, analysts construct the provenance graph to perform causality analysis on Point-Of-Interest (POI) event for capturing critical events (related to the attack). However, due to the vast size of the provenance graph and the rarity of critical events, existing attack investigation methods suffer from problems of high false positives, high overhead, and high latency. To this end, we propose SPARSE, an efficient and real-time system for constructing critical component graphs (i.e., consisting of critical events) from streaming logs. Our key observation is 1) Critical events exist in a suspicious semantic graph (SSG) composed of interaction flows between suspicious entities, and 2) Information flows that accomplish attacker's goal exist in the form of paths. Therefore, SPARSE uses a two-stage framework to implement attack investigation (i.e., constructing the SSG and performing path-level contextual analysis). First, SPARSE operates in a state-based mode where events are consumed as streams, allowing easy access to the SSG related to the POI event through semantic transfer rule and storage strategy. Then, SPARSE identifies all suspicious flow paths (SFPs) related to the POI event from the SSG, quantifies the influence of each path to filter irrelevant events. Our evaluation on a real large-scale attack dataset shows that SPARSE can generate a critical component graph (~ 113 edges) in 1.6 seconds, which is 2014 X smaller than the backtracking graph (~ 227,589 edges). SPARSE is 25 X more effective than other state-of-the-art techniques in filtering irrelevant edges.

==> bio.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/tiantian.eps}}]{Tiantian Zhu}

received the Ph.D. degree in computer science from Zhejiang University, Hangzhou, China, in 2019.
He is currently an associate professor with the college of computer science and technology, Zhejiang University of Technology, China. His research interests include mobile security, system security and artificial intelligence.

\end{IEEEbiography}

\vspace{-10mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/jiayu.eps}}]{Jiayu Wang}
received the B.E. degree in network engineering from Zhejiang University of Technology, Zhejiang, China, in 2019. He is currently studying for a master's degree in computer science at Zhejiang University of technology. His current research interests and directions include Cyberspace Security , APT attack detection and log analysis.

\end{IEEEbiography}

\vspace{-15mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/linqi.eps}}]{Linqi Ruan}

received her M.Eng. from Zhejiang university , Hangzhou, China, in 2020.She now is an assistant with the Department of Computer Science and Information Security, Zhejiang Police College, Hangzhou, China. Her research focuses on endpoint security and reverse engineering.

\end{IEEEbiography}

\vspace{-10mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/chunlin.eps}}]{Chunlin Xiong}

received his B.Eng. on computer science from Xian Jiaotong University, Xian, China, in 2015. He is currently a candidate of Ph.D. with the college of cyber security, Zhejiang University, China. His research interests include system security, software security and forensic analysis.

\end{IEEEbiography}

\vspace{-10mm}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/jinkai.eps}}]{Jinkai Yu}

received the B.E. degree in software engineering from Zhejiang University of Technology, Zhejiang, China, in 2019. He is currently pursuing M.S. degree for computer science in Zhejiang University of Technology. His current research interests include Cyberspace Security and APT.

\end{IEEEbiography}

\vspace{-10mm}




\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/yaosheng.eps}}]{Yaosheng Li}

received the B.E. degree in cyberspace security from Xi'an University of Posts & Telecommunications, Shanxi, China, in 2018. He is currently pursuing M.S. degree for computer science in Zhejiang University of Technology. His current research interests include network security and system security.

\end{IEEEbiography}

\vspace{-10mm}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/yan.eps}}]{Yan Chen}

received the Ph.D. degree in computer science from the University of California, Berkeley, CA, USA, in 2003. He is a Professor with the Department of Electrical Engineering and Computer Science, Northwestern University, Evanston, IL, USA. Based on Google Scholar, his papers have been cited over 7000 times and his h-index is 34. His research interests include network security, measurement, and diagnosis for large-scale networks and distributed systems. Prof. Chen won the Department of Energy (DoE) Early CAREER Award in 2005, the Department of Defense (DoD) Young Investigator Award in 2007, and the Best Paper nomination in ACM SIGCOMM 2010.

\end{IEEEbiography}

\vspace{-10mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/lvmingqi.eps}}]{Mingqi Lv}

received the Ph.D. degree in computer science from Zhejiang University, Hangzhou, China, in 2012. He is currently an associated professor with the college of computer science and technology, Zhejiang University of Technology, China. His research interests include spatiotemporal data mining and ubiquitous computing.

\end{IEEEbiography}


\vspace{-10mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/chentieming.eps}}]{Tieming Chen}

received the Ph.D. degree in computer software and theory from BeiHang University, Beijing, China, in 2011. He is now a professor with the college of computer science and technology, Zhejiang University of Technology, Hangzhou, China. He is also a member of IEEE and ACM. His research interests include cyberspace security and intelligence security.

\end{IEEEbiography}




